ConvCodeWorld: Benchmarking Conversational Code Generation in Reproducible Feedback Environments

Large language models (LLMs) have proven invaluable for code generation, particularly in interactive settings. However, existing code generation benchmarks fail to capture the diverse feedback encountered in multi-turn interactions, limiting our ability to evaluate LLMs in these contexts. To address this gap, we present a set of novel benchmarks that explicitly model the quality of feedback provided to code generation LLMs. Our contributions are threefold: First, we introduce CONVCODEWORLD, a novel and reproducible environment for benchmarking interactive code generation. CONVCODEWORLD simulates 9 distinct interactive code generation scenarios while systematically combining three types of feedback: (a) compilation feedback; (b) execution feedback with varying test coverage; (c) verbal feedback generated by GPT-4o with different levels of expertise. Second, we introduce CONVCODEBENCH, a fast, static version of benchmark that uses pre-generated feedback logs, eliminating the need for costly dynamic verbal feedback generation while maintaining strong Spearman's rank correlations (0.82 to 0.99) with CONVCODEWORLD. Third, extensive evaluations of both closed-source and open-source LLMs including R1-Distill on CONVCODEWORLD reveal key insights: (a) LLM performance varies significantly based on the feedback provided; (b) Weaker LLMs, with sufficient feedback, can outperform single-turn results of state-of-the-art LLMs without feedback; (c) Training on a specific feedback combination can limit an LLM's ability to utilize unseen combinations; (d) LLMs solve problems in fewer turns (high MRR) may not solve as many problems overall (high Recall), and vice versa. All implementations and benchmarks will be made publicly available at https://huggingface.co/spaces/ConvCodeWorld/ConvCodeWorld

==> fig/convcodebench_cumul_rank_correlation_deepseek_w_ref.tex <==
\begin{figure*}[t]
\centering
\hspace*{-0.5cm}
\begin{tabular}{ccc}
\subfloat[CF + EF (Public TCs) + SNF (Spearman's rank correlation=0.9286; P-value=0.0009)\label{fig:static_cf_ef_public_snf_deepseek_w_ref}]{%
      \includegraphics[width=0.31\linewidth]{fig/static_cumul_deepseek/CUMUL_CF_EF_PUBLIC_SNF.png}} 
& 
\subfloat[CF + EF (Full TCs) + SNF (Spearman's rank correlation=0.9524; P-value=0.0003)\label{fig:static_cf_ef_full_snf_deepseek_w_ref}]{%
      \includegraphics[width=0.31\linewidth]{fig/static_cumul_deepseek/CUMUL_CF_EF_FULL_SNF.pdf}}
&
\subfloat[CF + SEF (Spearman's rank correlation=0.8333; P-value=0.0102)\label{fig:static_cf_sef_deepseek_w_ref}]{%
      \includegraphics[width=0.31\linewidth]{fig/static_cumul_deepseek/CUMUL_CF_SEF.pdf}} \\
&
\hspace*{-5cm}
\subfloat[CF + EF (Public TCs) + SEF (Spearman's rank correlation=0.8095; P-value=0.0149)\label{fig:static_cf_ef_public_sef_deepseek_w_ref}]{%
      \includegraphics[width=0.31\linewidth]{fig/static_cumul_deepseek/CUMUL_CF_EF_PUBLIC_SEF.pdf}}
& 
\hspace*{-5cm}
\subfloat[CF + EF (Full TCs) + SEF (Spearman's rank correlation=0.7857; P-value=0.0208)\label{fig:static_cf_ef_full_sef_deepseek_w_ref}]{%
      \includegraphics[width=0.31\linewidth]{fig/static_cumul_deepseek/CUMUL_CF_EF_FULL_SEF.pdf}}\\
\end{tabular}
\caption{Rank correlation between Cumulative Pass@$1$ gain on \oursstatic (ref. DeepSeek-Coder-6.7B-Instruct) and Recall on \ourslive with different feedback combination. }
\label{fig:static_cumul_rank_correlation_deepseek_w_ref}
\end{figure*}

==> table/gt_code_leak.tex <==
\begin{table*}[htb!]
    \centering
    \caption{Recall results on \ourslive.} 
    \begin{tabular}{lccccccccccccccc}
        \thickhline
        \small Compilation Feedback & & \small \checkmark & \small \checkmark & \small \checkmark & \small \checkmark & \small \checkmark & \small \checkmark & \small \checkmark & \small \checkmark & \small \checkmark \\
        \small Execution Feedback & & & \small \checkmark & \small \checkmark & & \small \checkmark & \small \checkmark & & \small \checkmark & \small \checkmark \\ 
        \small Test cases & & &\scriptsize public &\scriptsize full & &\scriptsize public &\scriptsize full &  &\scriptsize public &\scriptsize full \\ 
        \small Simulated User Feedback & & & & & \small \checkmark & \small \checkmark & \small \checkmark & \small \checkmark & \small \checkmark & \small \checkmark \\ 
        \small User Expertise & & & & & \scriptsize novice & \scriptsize novice & \scriptsize novice & \scriptsize expert & \scriptsize expert & \scriptsize expert \\\hline
        \small GPT-4-0613 & 46.0 & 46.0 & \underline{60.3} & \textbf{70.5} & 46.0 & \textbf{61.9} & \textbf{72.5} & \textbf{89.7} & \textbf{91.1} & \textbf{92.5} \\
        \small GPT-4-Turbo-2024-04-09 & \underline{48.0} & \underline{48.0} & 56.7 & 63.8 & \underline{48.0} & 58.6 & 68.1 & \underline{84.7} & \underline{87.5} & \underline{88.5} \\
        \small GPT-4o-2024-05-13 & \textbf{50.8} & \textbf{50.8} & \textbf{60.5} & \underline{67.6} & \textbf{50.8} & \underline{60.8} & \underline{69.6} & 82.3 & 84.9 & 86.2 \\\hdashline
        \small DeepSeek-Coder-V2-Lite-Instruct & \underline{38.3} & \underline{38.3} & \textbf{43.4} & \textbf{46.1} & \underline{38.3} & \textbf{47.0} & \textbf{51.4} & 76.3 & 75.8 & 76.9 \\
        \small CodeQwen1.5-7B-Chat & \textbf{39.3} & \textbf{39.6} & \underline{40.1} & \underline{41.1} & \textbf{39.5} & \underline{45.8} & 49.5 & 74.4 & 74.7 & 77.4 \\
        \small CodeLlama-7B-Instruct-hf & 21.8 & 21.8 & 22.9 & 23.0 & 21.8 & 26.2 & 30.5 & 61.7 & 53.9 & 55.2 \\
        \small ReflectionCoder-DS-6.7B & 37.4 & 37.4 & 39.6 & 40.7 & 37.4 & 44.7 & \underline{50.4} & \underline{79.1} & \underline{79.6} & \underline{78.9} \\
        \small DeepSeek-Coder-6.7B-Instruct & 35.2 & 35.2 & 37.7 & 37.5 & 35.2 & 43.3 & 48.2 & \textbf{82.8} & \textbf{82.5} & \textbf{83.1} \\
        \thickhline
    \end{tabular}
    \label{tab:gt_code_leak}
\end{table*}



==> table/static_deepseek_cumul.tex <==
\begin{table*}[htb!]
    \centering
    \caption{CC-Recall on \oursstatic logs of DeepSeek-Coder-6.7B-Instruct in \ourslive. The dashed line separates the closed-source (above) and open-source (below) LLMs. For each column, Bold and underscore mean $1$st and $2$nd performance among the same source.\footnotemark[7]}
    \small
    \begin{tabular}{lccccccccccccccc}
        \thickhline
        \small Compilation Feedback & \small \cmark & \small \cmark & \small \cmark & \small \cmark & \small \cmark \\
        \small Execution Feedback & \small \cmark & \small \cmark & \xmark & \small \cmark & \small \cmark \\ 
        \small Test Coverage & \scriptsize part. &\scriptsize full &  &\scriptsize part. &\scriptsize full \\ 
        \small Simulated User Feedback & \small \cmark & \small \cmark & \small \cmark & \small \cmark & \small \cmark \\ 
        \small User Expertise & \scriptsize novice & \scriptsize novice & \scriptsize expert & \scriptsize expert & \scriptsize expert \\\hline
        \small GPT-4-0613 & 82.5 & \underline{131.0} & \underline{81.6} & \textbf{96.8} & \underline{99.5}\\
        \small GPT-4-Turbo-2024-04-09 & \underline{89.9} & 127.8 & 77.8 & 87.8 & 90.1\\
        \small GPT-4o-2024-05-13 & \textbf{96.0} & \textbf{132.7} & \textbf{82.9} & \underline{96.7} & \textbf{99.8}\\\hdashline
        \small DeepSeek-Coder-V2-Lite-Instruct & \textbf{24.5} & \phantom{0}\textbf{43.3} & \underline{47.2} & \textbf{57.8} & \textbf{55.1}\\
        \small CodeQwen1.5-7B-Chat & \underline{12.9} & \phantom{0}\underline{27.6} & 41.9 & \underline{47.4} & 45.4\\
        \small CodeLlama-7B-Instruct-hf & \phantom{0}6.4 & \phantom{0}10.3 & 33.9 & 39.3 & 32.2\\
        \small ReflectionCoder-DS-6.7B & 11.9 & \phantom{0}26.2 & 45.0 & 49.8 & 46.4\\
        \rowcolor{gray!10}
        \small DeepSeek-Coder-6.7B-Instruct (ref.) & \phantom{0}7.7 & \phantom{0}12.5 & \textbf{47.5} & 47.1 & \underline{47.8}\\
        \thickhline
    \end{tabular}
    \normalsize
    \label{tab:convcodebench_cumul_pass_gain_static}
\end{table*}

==> table/static_recall.tex <==
\begin{table*}[htb!]
    \subsection{C-Recall Results}
    \label{appendix:static_recall}
    \caption{C-Recall results on \oursstatic logs of DeepSeek-Coder-6.7B-Instruct in \ourslive. The dashed line separates the closed-source (above) and open-source (below) LLMs. For each column, Bold and underscore mean $1$st and $2$nd performance among the same source.\footnotemark[7]}
    \centering
    \small
    \begin{tabular}{lccccccccccccccc}
        \\
        \thickhline
        \small Compilation Feedback  & \small \cmark & \small \cmark & \small \cmark & \small \cmark & \small \cmark \\
        \small Execution Feedback & \small \cmark & \small \cmark & \xmark & \small \cmark & \small \cmark \\ 
        \small Test Coverage & \scriptsize part. &\scriptsize full &  &\scriptsize part. &\scriptsize full \\ 
        \small Simulated User Feedback & \small \cmark & \small \cmark & \small \cmark & \small \cmark & \small \cmark \\ 
        \small User Expertise & \scriptsize novice & \scriptsize novice & \scriptsize expert & \scriptsize expert & \scriptsize expert \\\hline
        \small GPT-4-0613 & \underline{61.8} & \textbf{68.9} & \textbf{89.9} & \textbf{90.6} & \textbf{91.0}\\
        \small GPT-4-Turbo-2024-04-09 & 61.7 & 68.3 & 89.0 & 89.9 & 90.0\\
        \small GPT-4o-2024-05-13 & \textbf{63.1} & \textbf{68.9} & \underline{89.8} & \underline{90.1} & \underline{90.5}\\\hdashline
        \small DeepSeek-Coder-V2-Lite-Instruct & \textbf{56.4} & \textbf{61.7} & \underline{86.2} & \textbf{87.1} & \textbf{87.7}\\
        \small CodeQwen1.5-7B-Chat & \underline{55.2} & \underline{60.8} & 86.1 & \underline{86.8} & \underline{87.4}\\
        \small CodeLlama-7B-Instruct-hf & 48.9 & 53.2 & \textbf{86.3} & 86.1 & 85.4\\
        \small ReflectionCoder-DS-6.7B & 52.5 & 56.9 & 85.8 & 85.9 & 86.4\\
        \rowcolor{gray!10}
        \small DeepSeek-Coder-6.7B-Instruct (ref.) & 43.3 & 48.2 & 82.8 & 82.5 & 83.1\\
        \thickhline
    \end{tabular}
    \normalsize
    \label{tab:convcodebench_recall_static}
\end{table*}

\begin{table*}[htb!]
    \centering
    \caption{C-Recall results on \oursstatic logs of CodeLlama-7B-Instruct-hf in \ourslive. The dashed line separates the closed-source (above) and open-source (below) LLMs. For each column, Bold and underscore mean $1$st and $2$nd performance among the same source.\footnotemark[7]}
    \small
    \begin{tabular}{lccccccccccccccc}
        \thickhline
        \small Compilation Feedback  & \small \cmark & \small \cmark & \small \cmark & \small \cmark & \small \cmark \\
        \small Execution Feedback & \small \cmark & \small \cmark & \xmark & \small \cmark & \small \cmark \\ 
        \small Test Coverage & \scriptsize part. &\scriptsize full &  &\scriptsize part. &\scriptsize full \\ 
        \small Simulated User Feedback & \small \cmark & \small \cmark & \small \cmark & \small \cmark & \small \cmark \\ 
        \small User Expertise & \scriptsize novice & \scriptsize novice & \scriptsize expert & \scriptsize expert & \scriptsize expert \\\hline
        \small GPT-4-0613 & 59.5 & 65.7 & 85.9 & \textbf{82.3} & 83.1\\
        \small GPT-4-Turbo-2024-04-09 & \underline{61.8} & \textbf{68.2} & \textbf{86.8} & 81.4 & \underline{84.2}\\
        \small GPT-4o-2024-05-13 & \textbf{62.1} & \underline{68.1} & \underline{86.2} & \underline{81.9} & \textbf{84.7}\\\hdashline
        \small DeepSeek-Coder-V2-Lite-Instruct & \textbf{51.1} & \textbf{55.6} & \textbf{82.0} & 74.7 & \underline{77.9}\\
        \small CodeQwen1.5-7B-Chat & \underline{49.1} & \underline{53.2} & 78.0 & 74.1 & 76.3\\
        \rowcolor{gray!10}
        \small CodeLlama-7B-Instruct-hf (ref.)  & 26.2 & 30.5 & 61.7 & 53.9 & 55.2\\
        \small ReflectionCoder-DS-6.7B & 46.7 & 51.6 & 79.3 & \underline{74.8} & 75.9\\
        \small DeepSeek-Coder-6.7B-Instruct & 46.8 & 52.9 & \underline{81.3} & \textbf{77.5} & \textbf{78.7}\\
        \thickhline
    \end{tabular}
    \normalsize
    \label{tab:convcodebench_recall_static_codellama}
\end{table*}

\begin{table*}[htb!]
    \caption{C-Recall results on \oursstatic logs of GPT-4-0613 in \ourslive. The dashed line separates the closed-source (above) and open-source (below) LLMs. For each column, Bold and underscore mean $1$st and $2$nd performance among the same source.\footnotemark[7]}
    \centering
    \small
    \begin{tabular}{lccccccccccccccc}
        \thickhline
        \small Compilation Feedback  & \small \cmark & \small \cmark & \small \cmark & \small \cmark & \small \cmark \\
        \small Execution Feedback & \small \cmark & \small \cmark & \xmark & \small \cmark & \small \cmark \\ 
        \small Test Coverage & \scriptsize part. &\scriptsize full &  &\scriptsize part. &\scriptsize full \\ 
        \small Simulated User Feedback & \small \cmark & \small \cmark & \small \cmark & \small \cmark & \small \cmark \\ 
        \small User Expertise & \scriptsize novice & \scriptsize novice & \scriptsize expert & \scriptsize expert & \scriptsize expert \\\hline
        \rowcolor{gray!10}
        \small GPT-4-0613 (ref.) & 61.9 & 72.5 & 89.7 & 91.1 & 92.5\\
        \small GPT-4-Turbo-2024-04-09 & \underline{67.2} & \underline{76.7} & \underline{91.6} & \underline{92.8} & \underline{94.2}\\
        \small GPT-4o-2024-05-13 & \textbf{68.6} & \textbf{77.2} & \textbf{91.9} & \textbf{93.0} & \textbf{94.3}\\\hdashline
        \small DeepSeek-Coder-V2-Lite-Instruct & \underline{66.4} & \underline{75.5} & 91.8 & 92.6 & 93.9\\
        \small CodeQwen1.5-7B-Chat & \textbf{67.1} & \textbf{76.1} & 91.8 & 92.9 & \textbf{94.4}\\
        \small CodeLlama-7B-Instruct-hf & 63.7 & 73.4 & \textbf{91.9} & 92.5 & 93.6\\
        \small ReflectionCoder-DS-6.7B & 65.7 & 75.2 & \textbf{91.9} & \underline{93.0} & 94.1\\
        \small DeepSeek-Coder-6.7B-Instruct & 65.7 & \underline{75.5} & 91.2 & \textbf{93.1} & \textbf{94.4}\\
        \thickhline
    \end{tabular}
    \normalsize
    \label{tab:convcodebench_recall_static_gpt4o}
\end{table*}


